ImitationFlow: Learning Deep Stable Stochastic Dynamic Systems by Normalizing Flows

We introduce ImitationFlow, a novel Deep generative model that allows learning complex globally stable, stochastic, nonlinear dynamics. Our approach extends the Normalizing Flows framework to learn stable Stochastic Differential Equations. We prove the Lyapunov stability for a class of Stochastic Differential Equations and we propose a learning algorithm to learn them from a set of demonstrated trajectories. Our model extends the set of stable dynamical systems that can be represented by state-of-the-art approaches, eliminates the Gaussian assumption on the demonstrations, and outperforms the previous algorithms in terms of representation accuracy. We show the effectiveness of our method with both standard datasets and a real robot experiment.

==> References.tex <==
On \cite{osa2018algorithmic}, Osa et al. made a taxonomy for policy representations. They categorize  the policies into three types : 1) task-level abstraction, 2) trajectory-level abstraction, and 3) action-state space abstraction. 

In task-level, the policy will learn to generate a sequence of a certain high level skills such as picking, go-to commands or dropping. In \cite{niekum2013incremental, Kroemer_ICRA_2014}, complex task were learned as a sequence of movement primitives.

Trajectory-level policies are also known as movement primitives. In this case, the learned policies will generate full state-action trajectories. Used mainly for \gls{bc}, several models arised . Deterministic models as \gls{dmp} \cite{schaal2006dynamic} or \gls{lwr} \cite{atkeson1997locally} or probabilistic models like \gls{promp}\cite{paraschos2013probabilistic} , \gls{seds} \cite{khansari2011learning} or \gls{kmp} \cite{huang2019kernelized}.

Finally, in action-state level, the learned policies maps a state with a control output, so on each instant a new control action is chosen depending on the current state. These type of policies are mainly used in \gls{irl} \cite{abbeel2004apprenticeship, finn2016guided, ho2016generative}, but also some \gls{bc} algorithms that learns nonlinear stable dynamic systems can lie in this category \cite{khansari2011learning,khansari2014learning}.





PPPPPPPPPPPPPPPPPPPPPPPPPPPPPPPP

Unlike time and time-state dependant movement primitives on which the control signal will provide a goal position that afterwards is tracked by a PID controller, in state-dependant movement primitives the attractor attitude should be provided by the model itself. Due to that, a good state dependant movement primitive should have stable dynamics towards a certain goal. 

In our work, we propose a deep stable dynamic model similar to \gls{seds} or \gls{clfdm}. ImitationFlows are able to represent not only point attractors but also limit cycles, outperforming the expressibility of other state dependant movement primitives. 


Imitation Flows are composed by two elements. Similar to \cite{perrin2016fast}, the motion evolves in a latent space in which some linear stable dynamics($A_{\phi}, \Sigma_{\phi}$) are imposed. Then, a diffeomorphic transformation($f_{\theta}$) is applied from the latent space to the space of our expert demonstrations.  The model is represented as graphical model in Figure \ref{im:ImitationFlow} and as mathematical representation in Equation \ref{eq:ImitationFlow}.


These architecture brings lot of interesting properties to our movement primitive. Most of the probabilistic movement primitives assume normal distribution on the expert demonstrations \cite{paraschos2013probabilistic,khansari2011learning}. However, as our noise is applied directly in the latent space and not in the trajectory space, the diffeomorphic transformation is also applied on the noise and so, we can express way more complex distributions.



